Dom, cars don't fly! -- Or do they? In-Air Vehicle Maneuver for High-Speed Off-Road Navigation

When pushing the speed limit for aggressive off-road navigation on uneven terrain, it is inevitable that vehicles may become airborne from time to time. During time-sensitive tasks, being able to fly over challenging terrain can also save time, instead of cautiously circumventing or slowly negotiating through. However, most off-road autonomy systems operate under the assumption that the vehicles are always on the ground and therefore limit operational speed. In this paper, we present a novel approach for in-air vehicle maneuver during high-speed off-road navigation. Based on a hybrid forward kinodynamic model using both physics principles and machine learning, our fixed-horizon, sampling-based motion planner ensures accurate vehicle landing poses and their derivatives within a short airborne time window using vehicle throttle and steering commands. We test our approach in extensive in-air experiments both indoors and outdoors, compare it against an error-driven control method, and demonstrate that precise and timely in-air vehicle maneuver is possible through existing ground vehicle controls.

==> contents/approach_backup.tex <==
\section{Approach}
\label{sec::approach}

In this section, we first define the in-air vehicle maneuver problem with airborne kinodynamic modeling. Then, we discuss the physics principles of why and how in-air vehicle maneuver is possible through existing vehicle controls, i.e., throttle and steering, based on the gyroscopic and inertial effects of the spinning wheels. 
Motivated by the difficulty in accurately and analytically modeling changing quantities purely based on physics, we present PHysics and Learning based model for In-air vehicle maneuver (\model, pronounced as ``fly''), a precise and efficient hybrid modeling approach. Finally, we introduce our \planner~(\textit{named after Dominic Toretto, who makes cars fly. So does our planner.})  for vehicle trajectory planning to reorient the robot from its current configuration to the goal precisely at when a limited airborne time window expires. 

\subsection{Problem Formulation}
We first formulate a discrete-time forward kinodynamic modeling problem based on a bicycle model, where the subsequent state, $\mathbf{s}_{t+1} \in \mathcal{S}$, is derived from the current state, $\mathbf{s}_t \in \mathcal{S}$, and current action, $\mathbf{a}_t \in \mathcal{A}$, with $\mathcal{S}$ and $\mathcal{A}$ as the state and action spaces respectively. Considering that during aerial phases a conventional ground vehicle does not have control over the three translational components in $\mathbb{SE}(3)$ (which is determined solely by gravity), we include in the vehicle state $\mathbf{s}_t$ a tuple of the three angles in $\mathbb{SO}(3)$, i.e., roll, pitch, and yaw, together with their corresponding angular velocities. We also include rotation per minute of the wheels, $\textrm{rpm}$, and the front steering angle, $\psi$, in the state space, i.e., $\mathcal{S} \subset \mathbb{R}^8$. The state at time $t$ is denoted as 
\begin{equation}
        \mathbf{s}_t = (\textrm{roll}_t, \dot{\textrm{roll}}_t, \textrm{pitch}_t, \dot{\textrm{pitch}}_t, \textrm{yaw}_t, \dot{\textrm{yaw}}_t, \textrm{rpm}_t, \psi_t) \in \mathcal{S}. \nonumber
\end{equation}

The vehicle action, $\mathbf{a}_t$, comprises the change rate in wheel $\textrm{rpm}$ (throttle) and in steering angle $\psi$, which are common controls available for ground robots. The action in the action space, $\mathcal{A} \subset \mathbb{R}^2$, is thus defined as a two-dimensional tuple:
\begin{equation}
    \begin{gathered}
        \mathbf{a}_t = (\dot{\textrm{rpm}}_t, \dot{\psi}_t) \in \mathcal{A}.
        \nonumber
    \end{gathered}
\end{equation}

A forward kinodynamics model is defined as a function, $f_{\theta}:\mathcal{S} \times \mathcal{A} \rightarrow \mathcal{S}$, parametrized by $\theta$, such that:
\begin{equation}
\mathbf{s}_{t+1} = f_{\theta}(\mathbf{s}_t, \mathbf{a}_t). 
\label{eqn::dynamics}
\end{equation}
% $f_{\theta}$ is subject to the constraint that the vehicle must attain a predefined goal state, $s^g \in \mathcal{S}$, corresponding to a controlled landing. 

After an aerial phase, the vehicle should land on the ground with an appropriate configuration. Unlike traditional navigation planning problems, in which the goal is to achieve a desired state with certain notion of minimal cost (shortest path, lowest energy, etc.), for our in-air maneuver problem the goal is to achieve a goal configuration precisely when a small airborne time window expires, i.e., the landing time, $T$. Therefore, the goal is to achieve: 
\begin{equation}
\mathbf{s}_T^g = (\textrm{roll}_T^g, \dot{\textrm{roll}}_T^g, \textrm{pitch}_T^g, \dot{\textrm{pitch}}_T^g, \textrm{yaw}_T^g, \dot{\textrm{yaw}}_T^g, \textrm{rpm}_T^g, \psi_T^g).  
\end{equation}
Notice that $\mathbf{s}_T^g$ must be achieved precisely at $T$, not later. If it is achieved at $t<T$, the vehicle needs to assure it maintains the same state at the landing time $T$. 
% The goal state is characterized by specific $\textrm{roll}$, $\textrm{pitch}$, and $\textrm{yaw}$ angles, denoted as $\textrm{roll}^g$, $\textrm{pitch}^g$, and $\textrm{yaw}^g$ respectively. 
For example, when the landing region is horizontal, $\textrm{roll}_T^g$ and $\textrm{pitch}_T^g$ become zero, while $\dot{\textrm{roll}}_T^g$ and $\dot{\textrm{pitch}}_T^g$ should be as close to zero as possible to minimize impact. $\textrm{yaw}_T^g$ and $\dot{\textrm{yaw}}_T^g$ are often less crucial since they do not cause significant impact during landing. $\textrm{rpm}_T^g$ mostly needs be positive to avoid flipping over the vehicle upon ground contact with forward momentum, and $\psi_T^g$ depends on what the immediate ground maneuver necessary for the vehicle to execute right after landing is, e.g., to quickly swerve to avoid an upcoming obstacle. 
% Crucially, the rates of change of $\textrm{roll}$, $\textrm{pitch}$, and $\textrm{yaw}$ must converge towards minimal values, approximating zero, to ensure a stable landing. Additionally, the goal state necessitates a positive rotational speed of the wheels, $rpm^g$, and a specific steering angle, $\psi^g$. Formally, the goal state is defined as:

Therefore, the in-air vehicle maneuver problem for safe landing can be formulated as 
\begin{equation}
    \begin{gathered}
    \mathbf{a}_0^*, ..., \mathbf{a}_{T-1}^* = \argmin_{\mathbf{a}_0, ..., \mathbf{a}_{T-1}} \sum_{t=0}^T c(\mathbf{s}_t, \mathbf{s}_T^g),\\
    \textrm{s. t.} \quad \mathbf{s}_{t+1} = f_\theta(\mathbf{s}_t, \mathbf{a}_t), \quad \mathbf{s}_0 \textrm{ is given}, \quad \textrm{and } \mathbf{s}_T = \mathbf{s}_T^g.
    \end{gathered}
\label{eqn::problem}
\end{equation}
$c$ is a state-wise cost function to be minimized, subject to the constraints by the forward kinodynamics, given initial state, and achieving the goal state at the end of the aerial phase $T$. Notice the difference of Problem~\eqref{eqn::problem} to traditional receding-horizon planning problems, where $T$ is a receding horizon which gradually moves towards the goal. Here $T$ is the end of the entire horizon of the problem, i.e., the landing point. 

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{contents/figures/Losi.png}
  \caption{Torques acting on the wheels and chassis due to wheel acceleration and steering.}
  \label{fig::torques}
  \vspace{-9pt}
\end{figure}

% Therefore, the learned transition function, $f$, is implicitly dependent on the action, $\mathbf{a}_t$, such that $\mathbf{s}_{t+1} = f_{\theta}(\mathbf{s}_t | \mathbf{a}_t)$. The learning problem can be formally stated as the determination of the functional relationship $f$, given a sequence of states and actions, subject to the constraint of achieving the goal state, $\mathbf{s}^g$. This framework enables the application of three different methods that we describe next.

% When the vehicle is in the air, we can change the state of the vehicle by leveraging 3 different methods:

\subsection{Physics Principles}
We discuss the physics principles of why and how in-air vehicle maneuver of $\mathbf{s}_{t+1}$ is possible with $\mathbf{a}_t = (\dot{\textrm{rpm}}_t, \dot{\psi}_t)$.

\subsubsection{Roll and Pitch Acceleration}

\paragraph{Zero-Steering Case ($\psi=0$)}

During aerial phases, the only external force acting on the vehicle is gravity (air resistance is overlooked for simplicity). Therefore, with a constant wheel speed, the vehicle maintains its angular momentum by the principle of conservation of angular momentum. 
All four wheels are rotating at the same speed, because the differentials will not differentiate left and right wheel speed due to the lack of ground contact. Therefore their combined angular momentum is given by
\begin{equation}
    L_{\textrm{all\_wheels}} = I_{\textrm{all\_wheels}} \cdot \omega,
    \nonumber
\end{equation}
where $I_{\textrm{all\_wheels}}$ is all wheels' combined moment of inertia along the chassis pitch axis, as combined from their individual wheel axles, and $\omega$ is their angular velocity.  

When the wheels are accelerated by applying a motor torque, the change in the wheels' angular velocity produces a change in angular momentum:
\begin{equation}
    % \begin{split}
     dL_{\textrm{all\_wheels}} = I_{\textrm{all\_wheels}} \cdot d \omega
     % dL_{\textrm{all\_wheels}} 
     = I_{\textrm{all\_wheels}}  \cdot d \textrm{rpm} \cdot \frac{2\pi}{60}.
    % \end{split}
     % \label{eq::dl_wheels_I_w}
     \nonumber
\end{equation}
% expressing change in angular velocity in terms of we write:
% \begin{equation}
%     d\omega = \dot{\textrm{rpm}} \cdot \frac{2\pi}{60} \cdot dt
% \end{equation}
As the angular momentum of the wheels increases due to this applied torque, the vehicle itself must gain an equal and opposite angular momentum to keep the net angular momentum of the body constant. 
This reaction to the wheels' torque results in a torque on the chassis of the vehicle $\tau_\textrm{chassis, pitch}$ that is equal in magnitude but opposite in direction:
\begin{equation}
    % \begin{split}
        \tau_\textrm{chassis, pitch} =  \frac{-dL_{\textrm{all\_wheels}}}{dt}.
    % \end{split}
% \label{eq::torque_chassis_to_rpm}
\nonumber
\end{equation}
$\tau_\textrm{chassis, pitch}$ can be used to exert control over the vehicle pitch: 
\begin{equation}
     \ddot{\textrm{pitch}} = \frac{\tau_\textrm{chassis, pitch}}{   I_{\textrm{chassis, pitch}}}, 
% \label{eq::torque_chassis}
\nonumber
\end{equation}
where $I_{\textrm{chassis, pitch}}$ is the moment of inertia of the chassis along the pitch axis. See Fig.~\ref{fig::torques} for a graphical illustration. 

\paragraph{Non-Zero-Steering Case ($\psi \neq 0$)}
% When the steering is turned to an angle $\psi$, with $\psi = 0$ being the wheels aligned with the vehicle's forward direction. 
With the wheels turned and accelerated, the change in angular momentum $dL_{\textrm{all\_wheels}}$ has components in both roll and pitch axes from the front wheels:
\begin{equation}
\begin{gathered}
        dL_{\textrm{all\_wheels}, \textrm{pitch}} = dL_{\textrm{front\_wheels}} \cdot cos (\psi) + dL_{\textrm{rear\_wheels}},\\
    % \label{eq::steering_pitch}
    % \nonumber
% \end{equation}
% \begin{equation}
        dL_{\textrm{all\_wheels}, \textrm{roll}} = dL_{\textrm{front\_wheels}} \cdot sin(\psi).
        % \label{eq::steering_roll}
        \nonumber
\end{gathered}
\end{equation}
% Accordingly, the reaction torques on the chassis are
% \begin{equation}
%     \tau_{\textrm{chassis}, \textrm{pitch}}=-I_{wheels} (\dot{\textrm{}{rpm}} \cdot \frac{2 \pi}{60})  \cdot cos(\theta)
%     \nonumber
%     \label{eq::tau_chasis_pitch_all}
% \end{equation}
% \begin{equation}
%     \tau_{\textrm{chassis}, \textrm{roll}}=-I_{wheels} (\dot{\textrm{}{rpm}} \cdot \frac{2 \pi}{60})  \cdot sin(\theta)
%     \nonumber
%     \label{eq::tau_chassis_roll_all}
% \end{equation}
Expressing the angular accelerations of the chassis by the torques on the pitch and roll axes, we have
\begin{equation}
\begin{gathered}
    \ddot{\textrm{pitch}} = \frac{- (I_\textrm{front\_wheels} \cdot cos(\psi) + I_\textrm{rear\_wheels}) \cdot 2 \pi }{I_{\textrm{chassis}, \textrm{pitch}} \cdot 60 } \cdot \dot{\textrm{rpm}},  \\
% \end{equation}
% \begin{equation}
    \ddot{\textrm{roll}} = \frac{- I_\textrm{front\_wheels}\cdot  sin(\psi) \cdot 2 \pi }{I_{\textrm{chassis}, \textrm{roll}} \cdot 60 } \cdot \dot{\textrm{rpm}}.
    \label{eqn::roll_dot_dot_1}
\end{gathered}
\end{equation}
Here $I_{\textrm{chassis}, \textrm{roll}}$ is the moment of inertia of the vehicle rotating along the roll axis.
% determined by the $\psi$ and $I_{\textrm{chassis}, \psi}$ = $I_{\textrm{chassis}, \textrm{pitch}}$ for $\psi= 0$.
We deduce that $\ddot{\textrm{pitch}}$ and $\ddot{\textrm{roll}}$ are directly proportional to $\dot{\textrm{rpm}}$ and dependent on the $sin$ or $cos$ component of the steering angle. We can leverage this property to maneuver vehicle roll and pitch in the air. 

\subsubsection{Precession for Roll}
Precession describes a phenomenon observed in spinning objects when an external torque is applied perpendicular to the spin axis.
This perpendicular torque causes a change in the axis of rotation and therefore angular momentum to rotate towards the axis of the applied torque while keeping the magnitude of the angular momentum constant.
This rotation of the spin axis is called precession.
For our case of in-air vehicle maneuver, the spinning object is the front wheels, and the external torque perpendicular to the wheel spin axis is from the steering servo to steer the front wheels. 

During in-air maneuvers, the front wheels spinning with angular velocity $\omega$ has angular momentum
\begin{equation}
    L = I_{\textrm{front\_wheels}} \cdot \omega \cdot \hat{z}_\textrm{front\_wheels}, 
    \nonumber
\end{equation}
where $I_{\textrm{front\_wheels}}$ is the front wheels' combined moment of inertia and $\hat{z}_\textrm{front\_wheels}$ is the unit vector equivalent of the front wheels' combined spin axis. 
When steering the wheel at a rate $\dot{\psi}$, the spin axis rotates towards the steering axis. This steering motion introduces a precession
\begin{equation}
    \Omega = \dot{\psi} \cdot \hat{z}_{\textrm{steering}}, 
    \nonumber
\end{equation}
% $\boldsymbol{\Omega}}$
where $\hat{z}_{\textrm{steering}}$ is the unit vector along the steering axis. 
The reaction torque on the vehicle chassis because of precession is determined by
\begin{equation}
% \tiny
    \tau_{\textrm{precession}} =  L \times \Omega \nonumber = I_{\textrm{front\_wheels}} \cdot \omega \cdot \hat{z}_\textrm{front\_wheels} \times \dot{\psi} \cdot \hat{z}_{\textrm{steering}}.
    \nonumber
\end{equation}
Since $\hat{z}_\textrm{front\_wheels}$ and $\hat{z}_{\textrm{steering}}$ are orthogonal, the magnitude of their cross product is 1 and the resultant direction is $\hat{z}_{\textrm{precession}}$ (see Fig.~\ref{fig::torques}). 
$\tau_{\textrm{precession}}$ has a component on both the roll and pitch axis:
\begin{align}
% \tiny
    \tau_{\textrm{precession}, \textrm{roll}} & = cos(\psi) \cdot \tau_{\textrm{precession}} = cos(\psi) \cdot I_{\textrm{front\_wheels}}  \cdot \omega \cdot \dot{\psi},\nonumber\\
    \tau_{\textrm{precession}, \textrm{pitch}} & = sin(\psi) \cdot \tau_{\textrm{precession}} = sin(\psi) \cdot I_{\textrm{front\_wheels}} \cdot \omega \cdot \dot{\psi}. \nonumber
\end{align}
% Since $\psi$ is usually small, $\hat{z}_{\textrm{roll}}$'s component on the pitch axis can be ignored, which makes it approximately only affect roll. 
% $\tau_{chassis, roll}$ can be simplified as
% \begin{equation}
%          \tau_{chassis, roll} = \dot{\psi} \cdot I_{\textrm{front\_wheels}} \cdot \omega  
% \end{equation}
Consequently $\ddot{\textrm{roll}}$ and $\ddot{\textrm{pitch}}$ can be derived as
\begin{align}
\small
    \ddot{\textrm{roll}} & = \frac{\tau_{\textrm{precession}, \textrm{roll}}}{I_{\textrm{chassis, wheel\_roll}}} = cos(\psi) \cdot \frac{I_{\textrm{front\_wheels}} \cdot \omega \cdot \dot{\psi}}{I_{\textrm{chassis, wheel\_roll}}} \nonumber\\
    &= cos(\psi) \cdot  \frac{I_{\textrm{front\_wheels}} \cdot 2\pi}{I_{\textrm{chassis, wheel\_roll}}\cdot 60} \cdot \textrm{rpm}\cdot \dot{\psi},\nonumber \\
    \ddot{\textrm{pitch}} & = \frac{\tau_{\textrm{precession}, \textrm{pitch}}}{I_{\textrm{chassis, wheel\_pitch}}} = cos(\psi) \cdot \frac{I_{\textrm{front\_wheels}} \cdot \omega \cdot \dot{\psi}}{I_{\textrm{chassis, wheel\_pitch}}} \nonumber\\
    &= cos(\psi) \cdot  \frac{I_{\textrm{front\_wheels}} \cdot 2\pi}{I_{\textrm{chassis, wheel\_pitch}}\cdot 60} \cdot \textrm{rpm}\cdot \dot{\psi},
    \label{eqn::roll_dot_dot_2}
\end{align}
where $I_{\textrm{chassis, wheel\_roll}}$ and $I_{\textrm{chassis, wheel\_pitch}}$ are the moment of inertia of the chassis along the front wheel's roll and pitch axis respectively. 
We deduce that $\ddot{\textrm{roll}}$ and $\ddot{\textrm{pitch}}$ are directly proportional to $\textrm{rpm}$ and $\dot{\psi}$. The final $\ddot{\textrm{roll}}$ and $\ddot{\textrm{pitch}}$ are a combined effect of both Eqns.~\eqref{eqn::roll_dot_dot_1} and \eqref{eqn::roll_dot_dot_2}. 

\subsubsection{Yaw Acceleration}
In theory, the vehicle action $\mathbf{a}_t = (\dot{\textrm{rpm}}_t, \dot{\psi}_t)$ does not have direct control over the yaw acceleration, $\ddot{\textrm{yaw}}$. But in practice, $\ddot{\textrm{yaw}}$ can be affected by system noises such as air resistance and weight distribution. Furthermore, initial yaw position, $\textrm{yaw}_0$, and yaw rate, $\dot{\textrm{yaw}}_0$, will still affect $\textrm{yaw}_t$ based on its inertia.  

\subsection{\model}
Calculating $\ddot{\textrm{roll}}$ and $\ddot{\textrm{pitch}}$ requires accurate moment of inertia measurements for the vehicle chassis and for the wheels.
These measurements are difficult to analytically derive or precisely measure due to changes in the center of gravity and weight distribution by steering and as a result of suspension movement.
Furthermore, expansion of the tires at high speeds due to centrifugal forces changes the moment of inertia of the wheels as well. 
Hence, we decompose the forward kinodynamics model $\mathbf{s}_{t+1} = f_{\theta}(\mathbf{s}_t, \mathbf{a}_t)$ into two parts, $g_\phi$ and $h_\xi$, i.e., $\mathbf{s}_{t+1} = h_\xi(g_{\phi}(\mathbf{s}_t, \mathbf{a}_t), \mathbf{s}_t, \mathbf{a}_t )$, and then employ a data-driven and a physics-based approach to derive $g_\phi$ and $h_\xi$ respectively. 

$g_\phi$ takes the state and action as input and derives the resultant acceleration of roll, pitch, and yaw
\begin{equation}
    \ddot{\textrm{roll}}_t, \ddot{\textrm{pitch}}_t, \ddot{\textrm{yaw}}_t = g_\phi(\mathbf{s}_t, \mathbf{a}_t),
\end{equation}
where model parameters $\phi$ are learned in a data-driven manner by minimizing a supervised loss. 
% The state $\mathbf{s}_t$ for this learned model is constructed from both raw and transformed variables. In our formulation, the input vector is defined as
% \begin{equation}
%     \begin{split}
%         \textbf{x}_t = [\textrm{rpm}_t, \psi_t, \sin(\textrm{roll}_t), \cos(\textrm{roll}_t), \sin(\textrm{pitch}_t),\\ 
%         \cos(\textrm{pitch}_t), \sin(\textrm{yaw}_t), \cos(\textrm{yaw}_t), \dot{\textrm{roll}}_t, \dot{\textrm{pitch}}_t, \dot{\textrm{yaw}}_t]
%     \end{split}
%     \nonumber
% \end{equation}
% and the action vector is given by $\textbf{u}_t = [\dot{\textrm{rpm}}_t,  \dot{\psi}_t ]$.
% The input to the supervised multilayer perception(MLP), is
% Thus, the full input to the supervised multilayer perceptron (MLP) is:
% \begin{equation}
%     \tilde{\mathbf{x}}_t = \Big[ \mathbf{x}_t,\; \mathbf{u}_t \Big].
%     \nonumber
% \end{equation}
% The target output is the angular acceleration vector:
% \begin{equation}
% \mathbf{y}_{t} = [ \ddot{\textrm{roll}}_{t+1},\; \ddot{\textrm{pitch}}_{t+1},\; \ddot{\textrm{yaw}}_{t+1}],
% \nonumber
% \end{equation}
The ground truth acceleration values are derived from the recorded Inertial Measurement Unit (IMU) data via differentiation over time.


Once $g_\phi$ is trained, its output angular accelerations are 
fed into $h_\xi$, along with the state $\mathbf{s}_t$ and action $\mathbf{a}_t$. For $\mathbf{s}_{t+1} = h_\xi((\ddot{\textrm{roll}}_t, \ddot{\textrm{pitch}}_t, \ddot{\textrm{yaw}}_t), \mathbf{s}_t, \mathbf{a}_t)$, we have
\begin{equation}
\begin{gathered}
    \dot{\textrm{roll}}_{t+1} = \dot{\textrm{roll}}_{t} + \ddot{\textrm{roll}}_t \cdot dt,\\
    \textrm{roll}_{t+1} = \textrm{roll}_{t} + \dot{\textrm{roll}}_t \cdot dt + \frac{1}{2} \ddot{\textrm{roll}}_t \cdot dt^2,\\
    \textrm{rpm}_{t+1} = \textrm{rpm}_{t} + \dot{\textrm{rpm}}_t \cdot dt,\\
    \psi_{t+1} = \psi_t + \dot{\psi}_t \cdot dt,
    \nonumber
\end{gathered}
\end{equation}
with analogous update equations for pitch and yaw. The only parameter for $h_\xi$ is the integration interval $dt$.  
This completes \model's transition to next state $\mathbf{s}_{t+1}$ given current state $\mathbf{s}_t$ and action $\mathbf{a}_t$ through $g_\phi$ and $h_\xi$. 

% \begin{figure}
%   \centering
%   \includegraphics[width=\columnwidth]{contents/figures/precession.jpeg}
%   \caption{Precession on a rotating wheel.}
%   \label{fig::precession}
%   \vspace{-9pt}
% \end{figure}

\subsection{\planner}
Given the short airtime, we adopt a fixed-horizon, instead of receding-horizon, planning approach, where the horizon is determined by the discretized time remaining until landing.
The planner samples action sequences over this fixed horizon and uses the learned \model~to rollout the corresponding state trajectories.
Each trajectory is then evaluated using a cost function. The planner selects the trajectory with the minimal cost, executes its first action, and replans with the updated (and reduced) remaining time. 
The next planning cycle samples around the best action from the last cycle. 
% This iterative re-planning naturally shortens the horizon over successive planning cycles.

One critical consideration of \planner~is that, in addition to general physical actuation limits (e.g., limited motor current and torque causing that the actions can never exceed certain thresholds), the under-actuated vehicle controls of $\dot{\textrm{rpm}}$ and $\dot{\psi}$ are further constrained due to state-dependent actuation limits:  
\begin{gather}
 \textrm{rpm}_\textrm{min} - \textrm{rpm}_t \leq \dot{\textrm{rpm}}_t^\textrm{feasible} \leq \textrm{rpm}_\textrm{max} - \textrm{rpm}_t, \nonumber \\
 \psi_\textrm{min} - \psi_t \leq \dot{\psi}_t^\textrm{feasible} \leq \psi_\textrm{max} - \psi_t,
 \nonumber
\end{gather}
which means if $\textrm{rpm}_t$ ($\psi_t$) is at the minimal value, $\dot{\textrm{rpm}}_t^\textrm{feasible}$ ($\dot{\psi}_t^\textrm{feasible}$) cannot be negative, and if $\dot{\textrm{rpm}}_t$ ($\psi_t$) is at the maximal value, $\dot{\textrm{rpm}}_t^\textrm{feasible}$ ($\dot{\psi}_t^\textrm{feasible}$) cannot be positive. 
This limited range of feasible $\dot{\textrm{rpm}}$ and $\dot{\psi}$ reduces possible in-air maneuver options and makes simple error-driven controllers, like PID controllers, inappropriate to enable complex in-air vehicle maneuvers. 

To enable goal convergence within a short aerial phase, the state-wise cost function defined in the fixed-horizon, instead of receding-horizon, problem in Eqn.~\eqref{eqn::problem} is formulated as:
\begin{align}
c(\mathbf{s}_t, \mathbf{s}_T^g) = \sum_{i=1}^K w_i(t) \cdot c_i(\mathbf{s}_t, \mathbf{s}_T^g),
\label{eq::cost_function}
\end{align}
which is a combination of the costs of $K$ state dimensions (in our case, $K=8$). A key difference from conventional state-wise cost function is that each state dimension is dynamically weighed by a weight term $w_i(t)$ as a function of time $t$. For example, for initial time steps, it is more important to quickly align the vehicle angles to prepare for a safe landing pose, while the focus will gradually shift to the angular velocities, wheel rpm, and steering components later on to ensure landing with minimal impact on the vehicle.   

% \begin{align}
%     c(\boldsymbol{\mathbf{s}}_{0:T}, \mathbf{s}_T^g) = &\quad w_1 c_\textrm{rpy}(\boldsymbol{\mathbf{s}}_{0:T}, \mathbf{s}_T^g) c_\textrm{time} (\boldsymbol{\mathbf{s}}_{0:T}) \nonumber \\ &+ w_2 c_{\dot{\textrm{r}}\dot{\textrm{p}}\dot{\textrm{y}}}(\boldsymbol{\mathbf{s}}_{0:T}, \mathbf{s}_T^g) c_\textrm{time} (\boldsymbol{\mathbf{s}}_{0:T})\nonumber \\ &+ w_3 c_{\textrm{rpm}} (\boldsymbol{\mathbf{s}}_{0:T}, \mathbf{s}_T^g) + w_4 c_{\psi}(\boldsymbol{\mathbf{s}}_{0:T}, \mathbf{s}_T^g) 
%     \label{eq::cost_function}
% \end{align}
% where $c_\textrm{rpy}(\cdot)$ and $c_{\dot{\textrm{r}}\dot{\textrm{p}}\dot{\textrm{y}}}(\cdot)$ are the costs for roll, pitch, and yaw and their first order derivatives. $c_\textrm{rpm}(\cdot)$ and $c_{\psi}(\cdot)$ are the respective costs for $\textrm{rpm}$ and $\psi$. Furthermore, $c_\textrm{time}(\cdot)$ penalizes trajectories based on the remaining time, incentivizing the planner to reach appropriate landing configurations close to $T$. The weights $\{w_i\}_{i=1}^4$ prioritize each cost term. \xuesu{can you write how c time works?}


Additionally, based on the sampled trajectory with the lowest cost, \planner~checks its feasibility of reaching the goal state within the time remaining till landing by computing the difference between the final state $\mathbf{s}_T$ and goal state $\mathbf{s}_T^g$. This feasibility check allows the system to either choose a viable trajectory or, if necessary, select an alternate goal to mitigate landing impact. 





